On LASSO for High Dimensional Predictive Regression

This paper examines LASSO, a widely-used $L_{1}$-penalized regression method, in high dimensional linear predictive regressions, particularly when the number of potential predictors exceeds the sample size and numerous unit root regressors are present. The consistency of LASSO is contingent upon two key components: the deviation bound of the cross product of the regressors and the error term, and the restricted eigenvalue of the Gram matrix. We present new probabilistic bounds for these components, suggesting that LASSO's rates of convergence are different from those typically observed in cross-sectional cases. When applied to a mixture of stationary, nonstationary, and cointegrated predictors, LASSO maintains its asymptotic guarantee if predictors are scale-standardized. Leveraging machine learning and macroeconomic domain expertise, LASSO demonstrates strong performance in forecasting the unemployment rate, as evidenced by its application to the FRED-MD database.

==> table/UNRATE_RMSE.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{center}
\caption{RMSPE for \texttt{UNRATE}}
\label{tab:unrate_RMSPE}
\small
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{cc|rcr|rr|rr|rr}
\hline\hline 
\multirow{2}{*}{$h$} & \multicolumn{1}{c|}{\multirow{2}{*}{$n$}} & \multicolumn{3}{c|}{Benchmarks}         & \multicolumn{2}{c|}{ST} & \multicolumn{2}{c|}{NT}                        & \multicolumn{2}{c}{LT}                       \\ \cline{3-11}
                   & \multicolumn{1}{c|}{}                   & \multicolumn{1}{r}{RW} & RWwD  & \multicolumn{1}{r|}{AR}    & \multicolumn{1}{r}{Plasso}    & \multicolumn{1}{r|}{Slasso}            & \multicolumn{1}{r}{Plasso} & \multicolumn{1}{r|}{Slasso} & \multicolumn{1}{r}{Plasso} & \multicolumn{1}{r}{Slasso} \\
                   \hline 
\multicolumn{11}{c}{\textbf{Entire testing sample: 1990--2019}}                                                                                                                                                                                                                            \\
 
\multirow{3}{*}{1} & 120 & 0.154 & 0.150 & 0.639 & \textit{0.144} & 0.889 & 0.511 & 0.578 & \textit{\textbf{0.139}} & 0.467 & 0.148                   \\
                   & 240 & 0.154 & 0.149 & 0.614 & \textit{0.145} & 0.632 & 0.647 & 0.766 & \textit{\textbf{0.128}} & 0.238 & 0.133                   \\
                   & 360 & 0.154 & 0.144 & 0.518 & \textit{0.150} & 1.864 & 1.920 & 0.736 & \textit{\textbf{0.129}} & 0.192 & 0.134                   \\
\multirow{3}{*}{2} & 120 & 0.230 & 0.214 & 0.689 & \textit{0.195} & 0.903 & 0.536 & 0.642 & \textit{\textbf{0.186}} & 0.556 & 0.204                   \\
                   & 240 & 0.230 & 0.205 & 0.821 & \textit{0.173} & 0.635 & 0.643 & 0.878 & \textit{\textbf{0.164}} & 0.303 & 0.176                   \\
                   & 360 & 0.229 & 0.199 & 0.600 & \textit{0.189} & 0.744 & 1.561 & 0.753 & \textit{\textbf{0.172}} & 0.255 & 0.176                   \\
\multirow{3}{*}{3} & 120 & 0.306 & 0.281 & 0.732 & \textit{0.266} & 0.953 & 0.563 & 0.710 & \textit{\textbf{0.264}} & 0.667 & 0.266                   \\
                   & 240 & 0.306 & 0.262 & 0.726 & \textit{0.242} & 0.641 & 0.654 & 1.011 & 0.245                   & 0.393 & \textit{\textbf{0.212}} \\
                   & 360 & 0.305 & 0.255 & 0.654 & \textit{0.225} & 0.741 & 1.177 & 0.786 & \textit{\textbf{0.213}} & 0.326 & 0.218                   \\

                    \hline 
                    \\
\multicolumn{11}{c}{Testing sub-sample:  1990--1999}                                                                                                                                                                                                                            \\
 
\multirow{3}{*}{1} & 120 & 0.141 & 0.138 & 0.469 & \textit{0.139} & 0.558 & 0.443 & 0.411 & \textit{\textbf{0.134}} & 0.258 & 0.143                   \\
                   & 240 & 0.141 & 0.138 & 0.204 & \textit{0.146} & 0.666 & 0.735 & 0.530 & \textit{\textbf{0.131}} & 0.193 & 0.133                   \\
                   & 360 & 0.141 & 0.141 & 0.221 & \textit{0.156} & 0.640 & 0.593 & 0.597 & 0.134                   & 0.181 & \textit{\textbf{0.131}} \\
                   \hline 
\multirow{3}{*}{2} & 120 & 0.189 & 0.180 & 0.483 & \textit{0.178} & 0.621 & 0.449 & 0.441 & \textit{\textbf{0.174}} & 0.294 & 0.184                   \\
                   & 240 & 0.189 & 0.184 & 0.266 & \textit{0.165} & 0.665 & 0.706 & 0.555 & \textit{\textbf{0.163}} & 0.269 & 0.175                   \\
                   & 360 & 0.190 & 0.187 & 0.272 & \textit{0.185} & 0.644 & 0.597 & 0.610 & \textit{\textbf{0.167}} & 0.244 & 0.168                   \\
                   \hline 
\multirow{3}{*}{3} & 120 & 0.234 & 0.224 & 0.503 & \textit{0.222} & 0.653 & 0.458 & 0.454 & \textit{\textbf{0.224}} & 0.340 & 0.233                   \\
                   & 240 & 0.234 & 0.226 & 0.393 & \textit{0.217} & 0.656 & 0.715 & 0.572 & \textit{\textbf{0.201}} & 0.338 & 0.212                   \\
                   & 360 & 0.237 & 0.229 & 0.336 & \textit{0.215} & 0.645 & 0.594 & 0.632 & 0.207                   & 0.307 & \textit{\textbf{0.200}} \\
                    \hline 
\multicolumn{11}{c}{Testing sub-sample: 2000--2009}                                                                                                                                                                                                                            \\
% \hline 
\multirow{3}{*}{1} & 120 & 0.168 & 0.150 & 0.439 & \textit{0.146} & 0.990 & 0.444 & 0.333 & \textit{\textbf{0.137}} & 0.648 & 0.149                   \\
                   & 240 & 0.169 & 0.145 & 0.663 & \textit{0.147} & 0.659 & 0.626 & 0.504 & \textit{\textbf{0.122}} & 0.236 & 0.122                   \\
                   & 360 & 0.169 & 0.141 & 0.388 & \textit{0.160} & 3.053 & 3.186 & 0.485 & \textit{\textbf{0.122}} & 0.197 & 0.123                   \\
                   \hline 
\multirow{3}{*}{2} & 120 & 0.282 & 0.237 & 0.576 & \textit{0.210} & 1.037 & 0.498 & 0.459 & \textit{\textbf{0.188}} & 0.700 & 0.225                   \\
                   & 240 & 0.283 & 0.219 & 1.105 & \textit{0.173} & 0.679 & 0.635 & 0.854 & \textit{\textbf{0.162}} & 0.282 & 0.174                   \\
                   & 360 & 0.282 & 0.212 & 0.515 & \textit{0.202} & 0.751 & 2.525 & 0.481 & 0.186                   & 0.269 & \textit{\textbf{0.174}} \\
                   \hline 
\multirow{3}{*}{3} & 120 & 0.399 & 0.333 & 0.652 & \textit{0.318} & 1.049 & 0.510 & 0.600 & \textit{\textbf{0.311}} & 0.718 & 0.313                   \\
                   & 240 & 0.400 & 0.305 & 0.709 & \textit{0.292} & 0.679 & 0.606 & 1.174 & 0.311                   & 0.310 & \textit{\textbf{0.212}} \\
                   & 360 & 0.399 & 0.293 & 0.555 & \textit{0.251} & 0.738 & 1.790 & 0.511 & 0.231                   & 0.334 & \textit{\textbf{0.228}} \\
                   \hline 
\multicolumn{11}{c}{Testing sub-sample: 2010--2019}                                                                                                                                                                                                                            \\
% \hline 
\multirow{3}{*}{1} & 120 & 0.151 & 0.160 & 0.902 & \textit{0.147} & 1.038 & 0.623 & 0.851 & \textit{\textbf{0.147}} & 0.408 & 0.151                   \\
                   & 240 & 0.150 & 0.163 & 0.806 & \textit{0.142} & 0.567 & 0.568 & 1.106 & \textit{\textbf{0.133}} & 0.278 & 0.145                   \\
                   & 360 & 0.149 & 0.151 & 0.779 & \textit{0.132} & 0.834 & 0.748 & 1.015 & \textit{\textbf{0.131}} & 0.199 & 0.146                   \\
                   \hline 
\multirow{3}{*}{2} & 120 & 0.208 & 0.221 & 0.926 & \textit{0.197} & 0.993 & 0.641 & 0.911 & \textit{\textbf{0.194}} & 0.592 & 0.200                   \\
                   & 240 & 0.207 & 0.210 & 0.855 & \textit{0.180} & 0.554 & 0.582 & 1.128 & \textit{\textbf{0.169}} & 0.352 & 0.180                   \\
                   & 360 & 0.204 & 0.197 & 0.861 & \textit{0.178} & 0.825 & 0.762 & 1.047 & \textit{\textbf{0.163}} & 0.250 & 0.185                   \\
                   \hline 
\multirow{3}{*}{3} & 120 & 0.259 & 0.274 & 0.964 & \textit{0.249} & 1.096 & 0.694 & 0.973 & 0.249                   & 0.839 & \textit{\textbf{0.246}} \\
                   & 240 & 0.257 & 0.248 & 0.962 & \textit{0.208} & 0.583 & 0.636 & 1.168 & \textit{\textbf{0.209}} & 0.502 & 0.213                   \\
                   & 360 & 0.253 & 0.240 & 0.928 & \textit{0.206} & 0.829 & 0.773 & 1.092 & \textit{\textbf{0.200}} & 0.335 & 0.225                                    \\
                   \hline \hline 
\end{tabular}
\end{center}
\footnotesize{Notes: ST, NT and LT are abbreviations for  stationarization transformation, no transformation and log-transformation, respectively. Bold numbers indicate the best performance in each row.}
\end{table}
